Node Query Preservation for Deterministic Linear Top-Down Tree Transducers

This paper discusses the decidability of node query preservation problems for XML document transformations. We assume a transformation given by a deterministic linear top-down data tree transducer (abbreviated as DLT^V) and an n-ary query based on runs of a tree automaton. We say that a DLT^V Tr strongly preserves a query Q if there is a query Q' such that for every document t, the answer set of Q' for Tr(t) is equal to the answer set of Q for t. Also we say that Tr weakly preserves Q if there is a query Q' such that for every t_d in the range of Tr, the answer set of Q' for t_d is equal to the union of the answer set of Q for t such that t_d = Tr(t). We show that the weak preservation problem is coNP-complete and the strong preservation problem is in 2-EXPTIME.

==> eptcsdata.tex <==
\providecommand{\firstpage}{27}
\providecommand{\publicationstatus}{S. Maneth (Ed.): Workshop on Trends in Tree\\
Automata and Tree Transducers (TTATT 2013).\\
EPTCS 134, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.134.4}{10.4204/EPTCS.134.4}}
\pdfoutput=1

